Estimation of the Sobolev embedding constant on domains with minimally smooth boundary

In this paper, we propose a method for estimating the Sobolev type embedding constant on a domain with minimally smooth boundary. We estimate the embedding constant by constructing an extension operator and computing its operator norm. We also present some examples of estimating the embedding constant for certain domains.

==> ref.tex <==
%% BioMed_Central_Bib_Style_v1.01

\begin{thebibliography}{21}
% BibTex style file: bmc-mathphys.bst (version 2.1), 2014-07-24
\ifx \bisbn   \undefined \def \bisbn  #1{ISBN #1}\fi
\ifx \binits  \undefined \def \binits#1{#1}\fi
\ifx \bauthor  \undefined \def \bauthor#1{#1}\fi
\ifx \batitle  \undefined \def \batitle#1{#1}\fi
\ifx \bjtitle  \undefined \def \bjtitle#1{#1}\fi
\ifx \bvolume  \undefined \def \bvolume#1{\textbf{#1}}\fi
\ifx \byear  \undefined \def \byear#1{#1}\fi
\ifx \bissue  \undefined \def \bissue#1{#1}\fi
\ifx \bfpage  \undefined \def \bfpage#1{#1}\fi
\ifx \blpage  \undefined \def \blpage #1{#1}\fi
\ifx \burl  \undefined \def \burl#1{\textsf{#1}}\fi
\ifx \doiurl  \undefined \def \doiurl#1{\textsf{#1}}\fi
\ifx \betal  \undefined \def \betal{\textit{et al.}}\fi
\ifx \binstitute  \undefined \def \binstitute#1{#1}\fi
\ifx \binstitutionaled  \undefined \def \binstitutionaled#1{#1}\fi
\ifx \bctitle  \undefined \def \bctitle#1{#1}\fi
\ifx \beditor  \undefined \def \beditor#1{#1}\fi
\ifx \bpublisher  \undefined \def \bpublisher#1{#1}\fi
\ifx \bbtitle  \undefined \def \bbtitle#1{#1}\fi
\ifx \bedition  \undefined \def \bedition#1{#1}\fi
\ifx \bseriesno  \undefined \def \bseriesno#1{#1}\fi
\ifx \blocation  \undefined \def \blocation#1{#1}\fi
\ifx \bsertitle  \undefined \def \bsertitle#1{#1}\fi
\ifx \bsnm \undefined \def \bsnm#1{#1}\fi
\ifx \bsuffix \undefined \def \bsuffix#1{#1}\fi
\ifx \bparticle \undefined \def \bparticle#1{#1}\fi
\ifx \barticle \undefined \def \barticle#1{#1}\fi
\ifx \bconfdate \undefined \def \bconfdate #1{#1}\fi
\ifx \botherref \undefined \def \botherref #1{#1}\fi
\ifx \url \undefined \def \url#1{\textsf{#1}}\fi
\ifx \bchapter \undefined \def \bchapter#1{#1}\fi
\ifx \bbook \undefined \def \bbook#1{#1}\fi
\ifx \bcomment \undefined \def \bcomment#1{#1}\fi
\ifx \oauthor \undefined \def \oauthor#1{#1}\fi
\ifx \citeauthoryear \undefined \def \citeauthoryear#1{#1}\fi
\ifx \endbibitem  \undefined \def \endbibitem {}\fi
\ifx \bconflocation  \undefined \def \bconflocation#1{#1}\fi
\ifx \arxivurl  \undefined \def \arxivurl#1{\textsf{#1}}\fi
\csname PreBibitemsHook\endcsname

%%% 1
\bibitem{aubin1976}
\begin{barticle}
\bauthor{\bsnm{Aubin}, \binits{T.}}:
\batitle{Probl\`emes isop\'erim\'etriques et espaces de {Sobolev}}.
\bjtitle{Journal of Differential Geometry}
\bvolume{11}(\bissue{4}),
\bfpage{573}--\blpage{598}
(\byear{1976})
\end{barticle}
\endbibitem

%%% 2
\bibitem{aubin1982book}
\begin{bbook}
\bauthor{\bsnm{Aubin}, \binits{T.}}:
\bbtitle{Nonlinear Analysis on Manifold. {Monge-Amp\`ere} Equations}.
\bpublisher{Springer},
\blocation{New York}
(\byear{1982})
\end{bbook}
\endbibitem

%%% 3
\bibitem{beckner1993}
\begin{barticle}
\bauthor{\bsnm{Beckner}, \binits{W.}}:
\batitle{Sharp {Sobolev} inequalities on the sphere and the {Moser--Trudinger}
  inequality}.
\bjtitle{Annals of Mathematics}
\bvolume{138}(\bissue{1}),
\bfpage{213}--\blpage{242}
(\byear{1993})
\end{barticle}
\endbibitem

%%% 4
\bibitem{brezis1983}
\begin{barticle}
\bauthor{\bsnm{Brezis}, \binits{H.}},
\bauthor{\bsnm{Nirenberg}, \binits{L.}}:
\batitle{Positive solutions of nonlinear elliptic equations involving critical
  {Sobolev} exponents}.
\bjtitle{Communications on Pure and Applied Mathematics}
\bvolume{36}(\bissue{4}),
\bfpage{437}--\blpage{477}
(\byear{1983})
\end{barticle}
\endbibitem

%%% 5
\bibitem{calderon1961}
\begin{bchapter}
\bauthor{\bsnm{Calder{\'o}n}, \binits{A.P.}}:
\bctitle{Lebesgue spaces of differentiable functions and distributions}.
In: \bbtitle{Proc. Sympos. Pure Math},
vol. \bseriesno{4},
pp. \bfpage{33}--\blpage{49}
(\byear{1961})
\end{bchapter}
\endbibitem

%%% 6
\bibitem{edmunds1987book}
\begin{bbook}
\bauthor{\bsnm{Edmunds}, \binits{D.E.}},
\bauthor{\bsnm{Evans}, \binits{W.}}:
\bbtitle{Spectral Theory and Differential Operators}.
\bpublisher{Oxford University Press},
\blocation{New York}
(\byear{1987})
\end{bbook}
\endbibitem

%%% 7
\bibitem{hestenes1941}
\begin{barticle}
\bauthor{\bsnm{Hestenes}, \binits{M.R.}}, \betal:
\batitle{Extension of the range of a differentiable function}.
\bjtitle{Duke Mathematical Journal}
\bvolume{8}(\bissue{1}),
\bfpage{183}--\blpage{192}
(\byear{1941})
\end{barticle}
\endbibitem

%%% 8
\bibitem{lieb1983}
\begin{botherref}
\oauthor{\bsnm{Lieb}, \binits{E.H.}}:
Sharp constants in the {Hardy-Littlewood-Sobolev} and related inequalities.
Annals of Mathematics,
349--374
(1983)
\end{botherref}
\endbibitem

%%% 9
\bibitem{nakao2001numerical}
\begin{barticle}
\bauthor{\bsnm{Nakao}, \binits{M.T.}}:
\batitle{Numerical verification methods for solutions of ordinary and partial
  differential equations}.
\bjtitle{Numerical Functional Analysis and Optimization}
\bvolume{22}(\bissue{3-4}),
\bfpage{321}--\blpage{356}
(\byear{2001})
\end{barticle}
\endbibitem

%%% 10
\bibitem{plum2001computer}
\begin{barticle}
\bauthor{\bsnm{Plum}, \binits{M.}}:
\batitle{Computer-assisted enclosure methods for elliptic differential
  equations}.
\bjtitle{Linear Algebra and its Applications}
\bvolume{324}(\bissue{1}),
\bfpage{147}--\blpage{187}
(\byear{2001})
\end{barticle}
\endbibitem

%%% 11
\bibitem{plum2008}
\begin{barticle}
\bauthor{\bsnm{Plum}, \binits{M.}}:
\batitle{Existence and multiplicity proofs for semilinear elliptic boundary
  value problems by computer assistance}.
\bjtitle{Jahresbericht der Deutschen Mathematiker Vereinigung}
\bvolume{110}(\bissue{1}),
\bfpage{19}--\blpage{54}
(\byear{2008})
\end{barticle}
\endbibitem

%%% 12
\bibitem{stein1970book}
\begin{bbook}
\bauthor{\bsnm{Stein}, \binits{E.}}:
\bbtitle{Singular Integrals and Differentiability of Functions}.
\bpublisher{Princeton University Press},
\blocation{New Jersey}
(\byear{1970})
\end{bbook}
\endbibitem

%%% 13
\bibitem{takayasu2013verified}
\begin{barticle}
\bauthor{\bsnm{Takayasu}, \binits{A.}},
\bauthor{\bsnm{Liu}, \binits{X.}},
\bauthor{\bsnm{Oishi}, \binits{S.}}:
\batitle{Verified computations to semilinear elliptic boundary value problems
  on arbitrary polygonal domains}.
\bjtitle{Nonlinear Theory and Its Applications, IEICE}
\bvolume{4}(\bissue{1}),
\bfpage{34}--\blpage{61}
(\byear{2013})
\end{barticle}
\endbibitem

%%% 14
\bibitem{talenti1976}
\begin{barticle}
\bauthor{\bsnm{Talenti}, \binits{G.}}:
\batitle{Best constant in {Sobolev} inequality}.
\bjtitle{Annali di Matematica pura ed Applicata}
\bvolume{110}(\bissue{1}),
\bfpage{353}--\blpage{372}
(\byear{1976})
\end{barticle}
\endbibitem

%%% 15
\bibitem{watanabe2009symmetrization}
\begin{barticle}
\bauthor{\bsnm{Watanabe}, \binits{K.}},
\bauthor{\bsnm{Kametaka}, \binits{Y.}},
\bauthor{\bsnm{Nagai}, \binits{A.}},
\bauthor{\bsnm{Yamagishi}, \binits{H.}},
\bauthor{\bsnm{Takemura}, \binits{K.}}:
\batitle{Symmetrization of functions and the best constant of 1-dim sobolev
  inequality}.
\bjtitle{Journal of Inequalities and Applications}
\bvolume{2009}(\bissue{1}),
\bfpage{874631}
(\byear{2009})
\end{barticle}
\endbibitem

%%% 16
\bibitem{whitney1934}
\begin{barticle}
\bauthor{\bsnm{Whitney}, \binits{H.}}:
\batitle{Analytic extensions of differentiable functions defined in closed
  sets}.
\bjtitle{Transactions of the American Mathematical Society}
\bvolume{36}(\bissue{1}),
\bfpage{63}--\blpage{89}
(\byear{1934})
\end{barticle}
\endbibitem

%%% 17
\bibitem{adams2003book}
\begin{bbook}
\bauthor{\bsnm{Adams}, \binits{R.A.}},
\bauthor{\bsnm{Fournier}, \binits{J.J.}}:
\bbtitle{Sobolev Spaces},
\bedition{2}nd edn.
\bsertitle{Pure and applied mathematics}.
\bpublisher{Academic Press},
\blocation{New York}
(\byear{2003})
\end{bbook}
\endbibitem

%%% 18
\bibitem{brezis2011book}
\begin{bbook}
\bauthor{\bsnm{Brezis}, \binits{H.}},
\bauthor{\bsnm{Br{\'e}zis}, \binits{H.}},
\bauthor{\bsnm{Brezis}, \binits{H.}}:
\bbtitle{Functional Analysis, {Sobolev} Spaces and Partial Differential
  Equations}.
\bpublisher{Springer},
\blocation{New York}
(\byear{2011})
\end{bbook}
\endbibitem

%%% 19
\bibitem{fraenkel1979}
\begin{barticle}
\bauthor{\bsnm{Fraenkel}, \binits{L.}}:
\batitle{On regularized distance and related functions}.
\bjtitle{Proceedings of the Royal Society of Edinburgh: Section A Mathematics}
\bvolume{83}(\bissue{1-2}),
\bfpage{115}--\blpage{122}
(\byear{1979})
\end{barticle}
\endbibitem

%%% 20
\bibitem{rump1999book}
\begin{bchapter}
\bauthor{\bsnm{Rump}, \binits{S.}}:
\bctitle{{INTLAB - INTerval LABoratory}}.
In: \beditor{\bsnm{Csendes}, \binits{T.}} (ed.)
\bbtitle{{Developments~in~Reliable Computing}},
pp. \bfpage{77}--\blpage{104}.
\bpublisher{Kluwer Academic Publishers},
\blocation{Dordrecht}
(\byear{1999}).
\bcomment{\url{http://www.ti3.tuhh.de/rump/}}
\end{bchapter}
\endbibitem

%%% 21
\bibitem{hardy1952book}
\begin{bbook}
\bauthor{\bsnm{Hardy}, \binits{G.H.}},
\bauthor{\bsnm{Littlewood}, \binits{J.E.}},
\bauthor{\bsnm{P{\'o}lya}, \binits{G.}}:
\bbtitle{Inequalities}.
\bpublisher{Cambridge university press},
\blocation{Cambridge}
(\byear{1952})
\end{bbook}
\endbibitem

\end{thebibliography}

\newcommand{\BMCxmlcomment}[1]{}

\BMCxmlcomment{

<refgrp>

<bibl id="B1">
  <title><p>Probl\`emes isop\'erim\'etriques et espaces de
  {Sobolev}</p></title>
  <aug>
    <au><snm>Aubin</snm><fnm>T</fnm></au>
  </aug>
  <source>Journal of Differential Geometry</source>
  <publisher>Lehigh University</publisher>
  <pubdate>1976</pubdate>
  <volume>11</volume>
  <issue>4</issue>
  <fpage>573</fpage>
  <lpage>-598</lpage>
</bibl>

<bibl id="B2">
  <title><p>Nonlinear analysis on manifold. {Monge-Amp\`ere}
  equations</p></title>
  <aug>
    <au><snm>Aubin</snm><fnm>T</fnm></au>
  </aug>
  <publisher>New York: Springer</publisher>
  <pubdate>1982</pubdate>
</bibl>

<bibl id="B3">
  <title><p>Sharp {Sobolev} Inequalities on the Sphere and the
  {Moser--Trudinger} Inequality</p></title>
  <aug>
    <au><snm>Beckner</snm><fnm>W</fnm></au>
  </aug>
  <source>Annals of Mathematics</source>
  <publisher>Annals of Mathematics</publisher>
  <series><title><p>Second Series</p></title></series>
  <pubdate>1993</pubdate>
  <volume>138</volume>
  <issue>1</issue>
  <fpage>213</fpage>
  <lpage>242</lpage>
</bibl>

<bibl id="B4">
  <title><p>Positive solutions of nonlinear elliptic equations involving
  critical {Sobolev} exponents</p></title>
  <aug>
    <au><snm>Brezis</snm><fnm>H</fnm></au>
    <au><snm>Nirenberg</snm><fnm>L</fnm></au>
  </aug>
  <source>Communications on Pure and Applied Mathematics</source>
  <publisher>Wiley Online Library</publisher>
  <pubdate>1983</pubdate>
  <volume>36</volume>
  <issue>4</issue>
  <fpage>437</fpage>
  <lpage>-477</lpage>
</bibl>

<bibl id="B5">
  <title><p>Lebesgue spaces of differentiable functions and
  distributions</p></title>
  <aug>
    <au><snm>Calder{\'o}n</snm><fnm>AP</fnm></au>
  </aug>
  <source>Proc. Sympos. Pure Math</source>
  <pubdate>1961</pubdate>
  <volume>4</volume>
  <fpage>33</fpage>
  <lpage>-49</lpage>
</bibl>

<bibl id="B6">
  <title><p>Spectral theory and differential operators</p></title>
  <aug>
    <au><snm>Edmunds</snm><fnm>DE</fnm></au>
    <au><snm>Evans</snm><fnm>WD</fnm></au>
  </aug>
  <publisher>New York: Oxford University Press</publisher>
  <pubdate>1987</pubdate>
</bibl>

<bibl id="B7">
  <title><p>Extension of the range of a differentiable function</p></title>
  <aug>
    <au><snm>Hestenes</snm><fnm>MR</fnm></au>
    <au><cnm>others</cnm></au>
  </aug>
  <source>Duke Mathematical Journal</source>
  <publisher>Duke University Press</publisher>
  <pubdate>1941</pubdate>
  <volume>8</volume>
  <issue>1</issue>
  <fpage>183</fpage>
  <lpage>-192</lpage>
</bibl>

<bibl id="B8">
  <title><p>Sharp Constants in the {Hardy-Littlewood-Sobolev} and Related
  Inequalities</p></title>
  <aug>
    <au><snm>Lieb</snm><fnm>EH</fnm></au>
  </aug>
  <source>Annals of Mathematics</source>
  <publisher>JSTOR</publisher>
  <pubdate>1983</pubdate>
  <fpage>349</fpage>
  <lpage>-374</lpage>
</bibl>

<bibl id="B9">
  <title><p>Numerical verification methods for solutions of ordinary and
  partial differential equations</p></title>
  <aug>
    <au><snm>Nakao</snm><fnm>MT</fnm></au>
  </aug>
  <source>Numerical Functional Analysis and Optimization</source>
  <publisher>Taylor \& Francis</publisher>
  <pubdate>2001</pubdate>
  <volume>22</volume>
  <issue>3-4</issue>
  <fpage>321</fpage>
  <lpage>-356</lpage>
</bibl>

<bibl id="B10">
  <title><p>Computer-assisted enclosure methods for elliptic differential
  equations</p></title>
  <aug>
    <au><snm>Plum</snm><fnm>M</fnm></au>
  </aug>
  <source>Linear Algebra and its Applications</source>
  <publisher>Elsevier</publisher>
  <pubdate>2001</pubdate>
  <volume>324</volume>
  <issue>1</issue>
  <fpage>147</fpage>
  <lpage>-187</lpage>
</bibl>

<bibl id="B11">
  <title><p>Existence and multiplicity proofs for semilinear elliptic boundary
  value problems by computer assistance</p></title>
  <aug>
    <au><snm>Plum</snm><fnm>M</fnm></au>
  </aug>
  <source>Jahresbericht der Deutschen Mathematiker Vereinigung</source>
  <publisher>Berlin: Georg Reimer, 1892-</publisher>
  <pubdate>2008</pubdate>
  <volume>110</volume>
  <issue>1</issue>
  <fpage>19</fpage>
  <lpage>-54</lpage>
</bibl>

<bibl id="B12">
  <title><p>Singular integrals and differentiability of functions</p></title>
  <aug>
    <au><snm>Stein</snm><fnm>EM</fnm></au>
  </aug>
  <publisher>New Jersey: Princeton University Press</publisher>
  <pubdate>1970</pubdate>
</bibl>

<bibl id="B13">
  <title><p>Verified computations to semilinear elliptic boundary value
  problems on arbitrary polygonal domains</p></title>
  <aug>
    <au><snm>Takayasu</snm><fnm>A</fnm></au>
    <au><snm>Liu</snm><fnm>X</fnm></au>
    <au><snm>Oishi</snm><fnm>S</fnm></au>
  </aug>
  <source>Nonlinear Theory and Its Applications, IEICE</source>
  <publisher>The Institute of Electronics, Information and Communication
  Engineers</publisher>
  <pubdate>2013</pubdate>
  <volume>4</volume>
  <issue>1</issue>
  <fpage>34</fpage>
  <lpage>-61</lpage>
</bibl>

<bibl id="B14">
  <title><p>Best constant in {Sobolev} inequality</p></title>
  <aug>
    <au><snm>Talenti</snm><fnm>G</fnm></au>
  </aug>
  <source>Annali di Matematica pura ed Applicata</source>
  <publisher>Springer</publisher>
  <pubdate>1976</pubdate>
  <volume>110</volume>
  <issue>1</issue>
  <fpage>353</fpage>
  <lpage>-372</lpage>
</bibl>

<bibl id="B15">
  <title><p>Symmetrization of Functions and the Best Constant of 1-DIM Sobolev
  Inequality</p></title>
  <aug>
    <au><snm>Watanabe</snm><fnm>K</fnm></au>
    <au><snm>Kametaka</snm><fnm>Y</fnm></au>
    <au><snm>Nagai</snm><fnm>A</fnm></au>
    <au><snm>Yamagishi</snm><fnm>H</fnm></au>
    <au><snm>Takemura</snm><fnm>K</fnm></au>
  </aug>
  <source>Journal of Inequalities and Applications</source>
  <pubdate>2009</pubdate>
  <volume>2009</volume>
  <issue>1</issue>
  <fpage>874631</fpage>
</bibl>

<bibl id="B16">
  <title><p>Analytic extensions of differentiable functions defined in closed
  sets</p></title>
  <aug>
    <au><snm>Whitney</snm><fnm>H</fnm></au>
  </aug>
  <source>Transactions of the American Mathematical Society</source>
  <publisher>JSTOR</publisher>
  <pubdate>1934</pubdate>
  <volume>36</volume>
  <issue>1</issue>
  <fpage>63</fpage>
  <lpage>-89</lpage>
</bibl>

<bibl id="B17">
  <title><p>Sobolev Spaces</p></title>
  <aug>
    <au><snm>Adams</snm><fnm>RA</fnm></au>
    <au><snm>Fournier</snm><fnm>JJ</fnm></au>
  </aug>
  <publisher>New York: Academic Press</publisher>
  <edition>Second</edition>
  <series><title><p>Pure and applied mathematics</p></title></series>
  <pubdate>2003</pubdate>
</bibl>

<bibl id="B18">
  <title><p>Functional analysis, {Sobolev} spaces and partial differential
  equations</p></title>
  <aug>
    <au><snm>Brezis</snm><fnm>H</fnm></au>
    <au><snm>Br{\'e}zis</snm><fnm>H</fnm></au>
    <au><snm>Brezis</snm><fnm>H</fnm></au>
  </aug>
  <publisher>New York: Springer</publisher>
  <pubdate>2011</pubdate>
</bibl>

<bibl id="B19">
  <title><p>On regularized distance and related functions</p></title>
  <aug>
    <au><snm>Fraenkel</snm><fnm>LE</fnm></au>
  </aug>
  <source>Proceedings of the Royal Society of Edinburgh: Section A
  Mathematics</source>
  <publisher>Cambridge Univ Press</publisher>
  <pubdate>1979</pubdate>
  <volume>83</volume>
  <issue>1-2</issue>
  <fpage>115</fpage>
  <lpage>-122</lpage>
</bibl>

<bibl id="B20">
  <title><p>{INTLAB - INTerval LABoratory}</p></title>
  <aug>
    <au><snm>Rump</snm><fnm>{S.M.}</fnm></au>
  </aug>
  <source>{Developments~in~Reliable Computing}</source>
  <publisher>Dordrecht: Kluwer Academic Publishers</publisher>
  <editor>Tibor Csendes</editor>
  <pubdate>1999</pubdate>
  <fpage>77</fpage>
  <lpage>-104</lpage>
  <note>\url{http://www.ti3.tuhh.de/rump/}</note>
</bibl>

<bibl id="B21">
  <title><p>Inequalities</p></title>
  <aug>
    <au><snm>Hardy</snm><fnm>GH</fnm></au>
    <au><snm>Littlewood</snm><fnm>JE</fnm></au>
    <au><snm>P{\'o}lya</snm><fnm>G</fnm></au>
  </aug>
  <publisher>Cambridge: Cambridge university press</publisher>
  <pubdate>1952</pubdate>
</bibl>

</refgrp>
} % end of \BMCxmlcomment

